Ubiquitous evaluation of layer potentials using Quadrature by Kernel-Independent Expansion

We introduce a quadrature scheme--QBKIX--for the high-order accurate evaluation of layer potentials associated with general elliptic PDEs near to and on the domain boundary. Relying solely on point evaluations of the underlying kernel, our scheme is essentially PDE-independent; in particular, no analytic expansion nor addition theorem is required. Moreover, it applies to boundary integrals with singular, weakly singular, and hypersingular kernels. Our work builds upon Quadrature by Expansion (QBX), which approximates the potential by an analytic expansion in the neighborhood of each expansion center. In contrast, we use a sum of fundamental solutions lying on a ring enclosing the neighborhood, and solve a small dense linear system for their coefficients to match the potential on a smaller concentric ring. We test the new method with Laplace, Helmholtz, Yukawa, Stokes, and Navier (elastostatic) kernels in two dimensions (2D) using adaptive, panel-based boundary quadratures on smooth and corner domains. Advantages of the algorithm include its relative simplicity of implementation, immediate extension to new kernels, dimension-independence (allowing simple generalization to 3D), and compatibility with fast algorithms such as the kernel-independent FMM.

==> algo.tex <==
\section{Algorithmic considerations\label{sec:algo}}

The general \qbkix algorithm for locating of expansions near the
boundary of the domain is given in \pr{alg:overview}.
We expand that algorithm in \pr{alg:main} and point out some
noteworthy comments about each step.

\LinesNotNumbered
\begin{algorithm}[t!]
  \algcaption{alg:main}{Setup and evaluation of \qbkix}{}
  %
  \DontPrintSemicolon
  \SetKwBlock{SubalgBlock}{\nl}{}
  \SetKw{Subalg}{\nl}
  \SetKw{cmmt}{--}
  %
  \SubalgBlock(Adaptively refine the boundary to resolve the boundary
  data.\nllabel{aln:adap}){

    \cmmt The adaptive refinement is done based on the boundary curve
    and the boundary data.\;
    %
    \cmmt We discretize the boundary using $q$-node \gl rule, where
    $q$ is typically 16. Therefore, the boundary curve and the
    boundary data are represented in \ordinal{q} order Legendre
    polynomial.\;
    %
    \cmmt We initially start by sampling the boundary using a
    user-defined number of panels (typically one).\;
    %
    \cmmt Then, we recursively split the panels until the
    interpolation error on the fine grid using the coarse-grid
    coefficients is within the prescribed absolute tolerance $\atol$
    (we choose $\atol=\sci{-11}$, unless mentioned otherwise).\;
    %
  }
  %
  \SubalgBlock(Balance the boundary panels such that the ratio of the
  arclength of neighboring panels is less than
  two.\nllabel{aln:balance}){
    %
    \cmmt The objective of this stage is to avoid constructing
    expansions in the near zone of neighboring panels, as it was
    remarked in \pr{ssc:err-float} and \pr{rmk:twotoone-balance}. }
  %

  \SubalgBlock(Locate expansions based on the geometry of the
  panel.\nllabel{aln:locate}){
    %
    \cmmt For each collocation point on the boundary panels a
    expansion is located with a center at distance $\delta$ from the
    boundary\;
    %
    \cmmt The distance of each expansion $\cen$ to its associated
    panel is chosen to be $\delta = 0.25 l$ where $l$ is the panel arc
    length (as discussed in \pr{ssc:err-float} and depicted in
    \pr{fig:center-dist})\;
    %
    \cmmt By choosing the distance $\delta$ other dimensions of the
    expansion (such as $\rc$ and $\rp$) are determined by using the
    preset ratios\emdash/for instance, $\rc=\re/3$, $\rp=8\rc$, and
    using $\re=\delta$\emdash/ as discussed in
    \pr{ssc:err-float,ssc:error-bounds}).  However, the error is not
    very sensitive to these parameters.
    %
    \cmmt Since the boundary is adaptively refined to resolve the
    boundary data, although not rigorously test, the arclength is of a
    panel is directly proportional to the distance of singularity to
    the panel $\tilde\rho$ and consequently $\rp/\rho$ is almost
    always less than one.
    %
  }
  %
  \SubalgBlock(Refine the boundary by a factor of four to ensure the
  checks are in accurate region of panels.\nllabel{aln:refine}){
    \cmmt We denote the original boundary panels by $\pi$ and the
    refined panels by $\pi_{f}$. Each $\pi$ is refined to four
    $\pi_f$.\;
    \cmmt See \pr{ssc:err-float} and \pr{rmk:twotoone-balance} for
    more discussion.\;
  }
  %
  \SubalgBlock(Evaluate the boundary integral on check points using
  the refined boundary.\nllabel{aln:eval-check}){
    \cmmt For moderate and large problems, we use a python
    implementation of the \ki FMM \cite{kifmm} for evaluation of the
    potential on the check points.\;
  }
  %
  \SubalgBlock(Compute the coefficients for each expansion using the
  check values.\nllabel{aln:compute}){
    \cmmt Given the potential on the check points, the density on the
    proxy point is computed by solving \pr{eqn:prx-to-chk}, where it
    is solve by computing the pseudo-inverse of $\linopd{Q}$, denoted
    by $\linopd{Q}^\dagger$.  Here we use SVD to compute
    $\linopd{Q}^\dagger$ using the prescribed relative tolerance,
    typically $\apinv=\sci{-9}$.  \;
    %
    \cmmt The decay in the spectrum of $\linopd{Q}$ and its effect on
    the \qbkix error is discussed in \pr{ssc:err-float}.\;
    %
    \cmmt For many of the kernels considered here, the matrix
    $\linop{Q}$ is scale-invariant and we only need to compute
    $\linopd{Q}^\dagger$ only once.\; }
  %
  \SubalgBlock(Evaluate the center back on the boundary collocation
  point and/or target points near to the boundary.\nllabel{aln:eval}){
    \cmmt Each target point, including the collocation on the boundary
    panels $\pi$ (see \lref{alg:main}{aln:refine} for definition), is
    associated with an expansion.  When the expansion coefficient is
    known, the potential at the target can be easily evaluated using
    \pr{eqn:localexp}.\;
    %
    \cmmt When the expansion is used as singular quadrature (i.e. to
    compute the integral in \pr{eqn:generic-den}), the targets are
    collation points on the boundary panels $\pi$. The map from the
    check potential to the target potential can be computed as a
    matrix and stored for fast evaluation.\;
    %
  }
\end{algorithm}

\begin{SCfigure}[1.4][!bt]
  \centering
  \setlength\figureheight{2in}
  \includegraphics[height=\figureheight]{param-reval}
  %

  \mcaption{fig:param-reval}{Error at different evaluation radii}{ The
    error for evaluation of a single expansion with various $\rp$ and
    $\re$ but fixed $\rc$ and $\rho$.
    The expansion is interpolating a harmonic function using Laplace
    \dl kernel.
    The singularity of the interpolated function is at $\rho=4$,
    and $\rc=.025\rho$.
    The $y$-axis shows the error for centers while the evaluation
    points move from $\re=0$ all the way to the proxy circle.
    The dotted lines are $\re = k \rc$ for $k=1,2,\text{ and } 3$.
    In practice we have no direct control on $\frac{\rp}{\rho}$
    and it is implied by the panel size \note[AR]{as mentioned above, in the experiments it is typically less than $.5$ }.
    Here we chose $\np=128$, and $\nc=2\np$; the trends are the same
    for lower $\np$ and $\nc$.
  }
\end{SCfigure}

\begin{figure}[!bt]
  \centering
  \small
  %sizes are used for subfigures
  \setlength\figureheight{2.2in}
  \setlength\figurewidth{2.2in}
  \includepgf{center-dist}
  %
  \mcaption{fig:center-dist}{Error vs. center and singularity
    distances}{The induced error for singularities and centers at
    various distances from the boundary.
    The boundary data is generated by putting a Laplace singularity at
    distance $\tilde\rho$ from the boundary\emdash/the singularity
    distance to the center of expansion is $\rho > \tilde \rho$.
    The density is solve directly and \qbkix is used only for
    evaluation.
    The error \note[AR]{infinity norm} is computed using the known
    solution corresponding to the boundary data.
    The left plot shows the errors for the case with fixed number of
    panels on the boundary (40 panels).
    The right plot shows the errors for adaptive refinement of the
    boundary.
    In the latter case, the boundary and the boundary data are
    resolved to $\atol=\sci{-11}$.
    We use $\np=64$, $\nc=2\np$, $\rp=8\rc$, and $\re=3\rc$.
    In both cases, the center of expansion is located based on the
    panel size.
  }
\end{figure}

As discussed in \Lref{alg:main}{aln:locate}, the distance of the
center of the expansion changes based on panel size.
This implies that other dimensions of the expansion also change for
each panel.
Nonetheless, we use a fixed relative geometry for
centers\emdash/i.e. $\re/\rc=3$ and $\rp/\rc=8$.
This has the beneficial side effect that the map from potential on
check points to expansion densities can be reused for many of the
kernels (see \Lref{alg:main}{aln:compute}).

Based on \pr{eqn:err-bound}, the error of each \qbkix is determined by
$\rc/\rho, \rc/\rp, \re/\rc$, and $\ech$.
The value of $\rc/\rho$ is deduced from the panel arc length and we
would like $\re/\rc$ to be as large as possible \note[AR]{to drive
  down error we need smaller $\ech$ and boundary refinement}.
Based on our experimentation, we use $\re/\rc=3$.
To investigate the effect of $\rc/\rp$, we construct expansions with
various $\rp$.
The error at different distances $\re$ are plotted in
\pr{fig:param-reval}.
From the plot we see that the highest accuracy at the edge of
evaluation radius $\re$ is achieved for $\rp/\rho \approx 0.2$ that is
equal to $8 \rc$ for this case.
This trend persist among other expansions we tested.

In contrast to QBX, increasing $\nc$ and/or $\np$ does not pollute the
result due to the filtering effect of the check to proxy operator
(discussed in \pr{ssc:err-float}).
The number of proxy points $\np$ only affects the first term in
\pr{eqn:err-bound}.
In our experiments $\np$ is chosen to be $16$ or $32$.
We have not discussed the effect of the number of check points (in
\pr{ssc:err-exact}, $\nc$ is assumed to be large).
Having more check points reduces the aliasing error and improve the
accuracy of the pseudo inverse and we opt for $\nc=2\np$.

As we mentioned above, the choice of $\apinv$ for pseudo inverse has
filtering effect and keeps the extrapolation in control we chose
$\apinv=\sci{-9}$.

The choice of the distance of the center of the expansion to the panel
(relative to the panel size) is to balance the error due to evaluation
of smooth quadrature at the check points against the expansion's
interpolation error\emdash/for larger $\rc$ the singularity is
relatively closer.
This is shown in \pr{fig:center-dist}.
In all cases, as the expansions are placed farther from the boundary,
the error initially decreases due to the fact that the check points
move to more accurate regions of the domain.
But as the expansions move farther, they become larger and the
singularity gets close to them (relative to check and proxy radii) and
expansion's error dominate.
In both cases, the lowest error is achieved for $\delta/l \approx
0.25$.
When the boundary is adaptively refined (the right graph in
\pr{fig:center-dist}), the panel size changes depending on the
distance of singularity $\tilde\rho$.
Due to this, we have consistent error for different singularity
distances.

\begin{remark}
  \label{rmk:amortize}
  \note[AHB]{move to later near end of paper; too detailed here.} \note[AR]{I think now we have enough info before this}
  We associate with each collocation point on the boundary a single
  center with its own set of check points.
  One could try use less number of centers by associating more points
  with each center.
  One can try using less number of check points by reusing the check
  points of a centers in neighboring centers.
  We did not pursue such enhancements in this paper because they do
  not change the asymptotic complexity of evaluation steps.
\end{remark}

\begin{remark}
  If they are needed, derivatives of the solution can be evaluated
  after the construction of the expansion by differentiating the
  expansion basis.
\end{remark}

\para{Computational complexity of~\qbkix} Consider a domain with $M$
panels and $q$-node \gl discretization of the panels.
There are $N=Mq$ collocation points on the boundary.
Using FMM, the evaluation of the boundary integral from the refined
boundary to the check points is \O{4N \nc}.
The pseudo-inverse for computing the density can be precomputed and
applied as a matrix multiply with total cost of \O{k(\nc+\np)N}.
Each expansion is evaluated at its associated boundary collocation
point with total cost of \O{N\np}.
Therefore, the cost of one evaluation (e.g. in the context of
iterative solver) is \O{(4\nc + k\nc + k\np + \np)N}.
And with the choice of $\nc=2\np$, \O{(9 + 3k)\np N}.
This cost can be amortized if more targets are associated with each
expansion (see \pr{rmk:amortize}).
\note[AR]{It seems to me that this is dimension independent, of course $\np$ is greater for 3D}
\note[AHB]{Have we decided CPU time is irrelevant for this paper?
Can some comment be made about it being manageable? or a single timing
quoted to reassure the worried reader who wants to implement this?
}


==> overview.tex <==
\section{Overview of \qbkix\label{sec:overview}}
\begin{SCfigure}[1.4][!bt]
  \centering
  \small
  \setlength\figureheight{2.4in}
  \includepgf{schematic}
  %\includegraphics[width=4in,center]{geom}
  %
  \mcaption{fig:schematic}{Schematic of a \ki expansion}{Geometry of
    \qbkix\, showing the expansion centered at $\cen$ near a panel of
    the boundary $\Gamma$ discretized with $q$-node \gl rule.
    The points on which the solution is evaluated at are referred to
    as check points\emdash/the smooth quadrature (or a refined version
    of it) is used to evaluate the solution at check points.
    The check points are organized on a circle with radius $\rc$
    around the center of expansion $\cen$.
    A set of sources is located on a set of proxy points with radius
    $\rp$ around the center.
    Based on the desired accuracy, the expansion can be evaluated,
    within a permissible radius $\re$ away from $\cen$.
    For error analysis, the underlying solution is assumed to have a
    singularity at distance farther than $\rho$ from the center of the
    expansion.
    Note that, to better demonstrate different parts of \qbkix, the
    schematic is not plotted to scale.
  }
\end{SCfigure}

In \pr{fig:schematic}, we show the general geometry of a \ki expansion.
We use the term \emph{check points} to denote the set of points on
which the function can be evaluated accurately by the smooth
quadrature (or a refinement of it, we will clarify this in
\pr{sec:refinement}).
These points are organized on a circle with radius $\rc$.
The fundamental solutions of the PDE are located on the \emph{proxy
  points} to form the basis of the interpolation.
  The names check and proxy points are borrowed from the fast direct
  solvers \cite{Mart05,Corona2015a} and \ki FMM \cite{kifmm}, due to
  the similarity of the \ki expansion center here to the local
  expansion in the \ki FMM.
More formally, we let
\begin{alignln}
  \label{eqn:localexp}
  \ui(\vx) = \sum_{j=0}^{\np} \scalard{\alpha}_j \fundsol(\vx,\vy_j),
\end{alignln}
where $\vy_j~(\range[\np]{j})$ are the proxy points, $\fundsol$ is the
fundamental solution of $\op{L}$, and $\np$ is the number of proxy
points.
The proxy points are organized over a circle with radius $\rp$.
The values of function on the check points are used to determine the
expansion coefficients $\scalard{\alpha}_j~(\range[n_p]{j})$, namely
by solving the least-square problem.
Letting $\ud_i$ be known data at the check point $\vx_i$, then we
solve the least square problem
\begin{alignln}
  \vectord{\alpha} = \arg \min_{\vectord{\alpha}} \sum_{i=1}^{n_c} \left|
  \ui(\vx_i) - \ud_i \right|^2 = \arg \min_{\vectord{\alpha}}
  \sum_{i=1}^{n_c} \left| \sum_{j=1}^{n_p} \scalard{\alpha}_i
  \Phi(\vx_i,\vy_j) - \ud_i \right|^2.
\end{alignln}
We consider the boundary data $\scalar{f}$ and the curve $\Gamma$ to
be analytic, so that the density $\scalar{\phi}$ is also analytic.
In this case, $\u$ may be continued \emph{outside} $\Omega$ as a PDE
solution, at least to some open neighborhood of $\Omega$, but may have
singularities in $\R^2 \backslash \overline{\Omega}$ some positive
distance from $\Gamma$.
These singularities will control the exponential convergence rate
of local quadrature schemes \cite{ATAP,austinrou,ce} \note[AR]{and the \ki expansion}.
Therefore, for error analysis, we assume that the solution has
singularity at a distance farther than $\rho$ from the center of
expansion $\cen$.
In the case of merely smooth data, the convergence is expected to be
similar \note[AR]{similar to what?}.

To construct high-accuracy evaluator for the low accuracy region near
the panel as well as on the collocation points on the panel
$\vy_k~(\range[q]{k})$ we construct an expansion around a center
$\cen$ located near each collocation point, associate that expansion
with the collocation point on the boundary, and use the expansion at
$\cen$ to evaluate the integral at $\vy_k$.

Based on the geometry of the expansion (i.e. ratio of proxy radius to
check radius $\frac{\rp}{\re}$) and the desired evaluation accuracy
$\acc$, there is a maximum relative radius $\frac{\re}{\rc}$ from
$\cen$ where the expansion has error less than $\acc$. We denote this
radius by \emph{evaluation radius} $\re$.
The center is located such that $|\vy_k - \cen|=\re$ so that the
expansion can be evaluated at the associated boundary node.
Based on the value $\re$, some of the check points typically fall in
the inaccurate region of the smooth quadrature of the panel or that of
the neighboring panels.
To find accurate values of the solution $\ud$ on the checkpoint, the
boundary is split (or refined) into smaller panels, each with the same
$q$ nodes as the original panel (in all cases in this paper, into four
panels).
This also requires interpolating a known density $\scalard{\phi}$ onto
the new nodes, for which Lagrange interpolation on the original panel
is used.

The boundary could alternatively be upsampled, but for simplicity we
kept the order of panels fixed and split the panels.
After the expansions are constructed, i.e. it geometry is decided and
the expansion coefficients are computed, they are used to evaluate for
the targets that fall within their evaluation radius, including the
associated boundary point.
The main construction and evaluation steps of a \qbkix center is
depicted in \pr{fig:stages}.
\begin{figure}[!bt]
  \centering
  \small
  \setlength\figureheight{1.4in}
  \setlength\figurewidth{1.7in}
  \includepgf{error-stages}
  %
  \mcaption{fig:stages}{Stages of \qbkix construction}{An expansion is
    placed near the boundary at a distance proportional to the panel
    size.
    In order to evaluate the solution at the check point accurately,
    the boundary is refined.
    Using the values on the check point, an expansion is computed at
    the center (\pr{eqn:localexp}).
    The expansion is used for evaluation at all the points that fall
    within the center's evaluation radius.
    Most importantly, the associated point on the boundary is within
    the evaluation disc of the center.
    In this example Laplace \dl integral with constant density is
    used.
  }
\end{figure}

\begin{remark}
  As it was hinted in the previous paragraph and will be shown in
  \pr{sec:error}, the \ki expansion error at a distance from $\cen$
  depends on the relative geometry of the expansion ($\frac{\rc}{\rp}$,
  $\frac{\rp}{\rho}$, and $\frac{\re}{\rc}$).
  Ideally, the check radius should be as small as possible compared to
  $\rho$ (which is not known in practice).
  But, the small $\rc$ implies small $\re$ and causes excessive
  refinement of the boundary to get accurate data on the check points.
  We use the panel size as a surrogate for $\rho$ as the corrolate
  closely and decide a geometry for the expansion that balances these
  two errors (i.e. truncation error of expansion vs. extrapolation
  error).
\end{remark}

\begin{remark}
  The structure and construction of the \qbkix centers are very
  similar to the local expansions in the \ki FMM context.
  When used in conjunction with the \ki FMM, the local expansions can
  be used to speed up the construction of the \qbkix centers.
\end{remark}

\begin{remark}
  \qbkix centers can be categorized as global and local centers:
  \vspace{.5em}
  \begin{compactitem}
  \item \lhb{Global centers} are centers that interpolate the integral
    from all boundary panels \cite{QBX,Rachh2016}.
  \item \lhb{Local centers} are centers that interpolate the integral
    from a subset of boundary panels \cite{Rachh2016b}.
  \end{compactitem}
  \vspace{.5em}
  When the boundary is geometrically complicated, it is more efficient to use local
  centers \missingitem[cite Manas local].
  In this paper we focus on the construction and analysis of global
  \qbkix centers and postpone the extension of this work to local
  expansion centers to a later work.
\end{remark}

\begin{algorithm}
  \algcaption{alg:overview}{Overview of \qbkix}{\note[AR]{we have an
      expanded version in \pr{alg:main}; I think it's better to
      keep this simple}\note[AHB]{maybe add the equation references,
      or repeat the key equations there. E.g. step 6 requires the
      backward-stable soln of small dense ill-cond lin sys.}}
  %
  \DontPrintSemicolon
  %
  Adaptively refine the boundary to resolve the boundary data.\;
  %
  Balance the boundary panels such that the ratio of the arclength of
  neighboring panels is less than two.\;
  %
  Locate centers based on the geometry of the panel.\;
  %
  Refine the boundary by a factor of four to ensure the checks are in
  accurate region of panels.\;
  %
  Evaluate the boundary integral on check points using the refined
  boundary.\;
  %
  Compute each center's expansion coefficients using the check
  values.\;
  %
  Evaluate the center back on the boundary collocation point.\;
\end{algorithm}

\note[AHB]{Can you now write out full equations, or expand on Alg 1?}

